Geometric Hyena Networks for Large-scale Equivariant Learning

Processing global geometric context while preserving equivariance is crucial when modeling biological, chemical, and physical systems. Yet, this is challenging due to the computational demands of equivariance and global context at scale. Standard methods such as equivariant self-attention suffer from quadratic complexity, while local methods such as distance-based message passing sacrifice global information. Inspired by the recent success of state-space and long-convolutional models, we introduce Geometric Hyena, the first equivariant long-convolutional model for geometric systems. Geometric Hyena captures global geometric context at sub-quadratic complexity while maintaining equivariance to rotations and translations. Evaluated on all-atom property prediction of large RNA molecules and full protein molecular dynamics, Geometric Hyena outperforms existing equivariant models while requiring significantly less memory and compute that equivariant self-attention. Notably, our model processes the geometric context of 30k tokens 20x faster than the equivariant transformer and allows 72x longer context within the same budget.

==> rebuttal_mangal.tex <==
Reviewer YW9h:

1. I believe non-equivariant methods are included in the recall experiment, but not in the RNA experiments. It would be nice to see how they compare, for example, with ample data augmentation. Non-equivariant methods can often perform well too, especially when controlling for memory/compute budget which a focus of the current work.


2. Many of the local equivariant methods are targeted more for smaller scale material science tasks, so while they are good to include as baselines, it may not be surprising they do worse on these larger scale tasks with sequence structure. Is there some way to encode the sequence structure for these models? 

3. Also, although it is not the goal, I wonder how well would Geometric Hyena perform on the types of materials benchmarks those baselines target.


4. The higher order generalization is quite elegant and I suppose only did not make it into the main since the added complexity was not justified by any improvement in results. Where the higher order methods tested?


5. It is a bit unusual to not include a background section or related works section on prior works. That said, I think the narrative and explanation is clear and that past work and current contributions are clear as written.

6. Shouldn’t the input and output spaces for be the N-fold product of these spaces?
7. I found this a touch confusing. Are they sequences of sets of scalars? Maybe if the index i is across a sequence, you could use parenthesis instead of curly braces to indicate the order matters.
8. Why is the equivariant projection layer called a “projection”? Isn’t it just a mapping?

9. Is the Fourier transform truncated at some maximum frequency? If so, does it matter where
10. Does this scalar mapping result in a lot of lost information?
11. Are there any trade-offs with omitting some message pathways this way?
12. How big is the sequence length for the protein task? What is the input feature for the model?


Response: 

We thank the reviewer for their invaluable comments and strong endorsement of the novelty and the practical importance of our G-Hyena architecrure for multiple real-world biomolecular tasks. Below we answer the questions point-by-point.

**1. Inclusion of Non-Equivariant Methods in Experiments:** Thank you for the insightful point! Following your suggestion, we have now run the vanilla non-equivariant Hyena for RNA property prediction and protein MD tasks. Below, we summarize our results, which show that GHyena outperforms the non-equivariant counterparts on all tasks, with improvements ranging from 3% to 875%, depending on the task.

**2. Encoding Sequence Structure in Local Equivariant Methods:** Thank you for the suggestion! Incorporating sequence structure is akin to encoding global context for local models and is indeed a useful research direction. Recent works, such as FastEGNN and LeftNet, have attempted to address this using techniques like virtual nodes and learning global information from local patches, respectively. For this reason, we have already included FastEGNN and LeftNet as baselines in our evaluations, which still underperform compared to GHyena on all datasets considered. Nonetheless, we agree that further exploration in this area would be a valuable future research direction.

**3. Performance of GHyena on Materials Benchmarks:** This is a great suggestion! We believe that GHyena could be useful for materials benchmarks as well. However, since we are not yet familiar with these benchmarks sicne we do not work in this area, we did not run the models on them, as it would require time to understand the benchmark tasks and familiarize ourselves with the data. Nonetheless, we are confident that GHyena can stimulate further research in this important field and inspire researchers to consider similar models for materials.

**4. Testing of Higher Order Generalization:**

**5. Related Works Section In Main Text:** We included the related works in the Appendix A due to page limitations. We followed the examples of prior works accepted at NeurIPS, ICML, and ICLR, which also compiled the related work in the appendix [1, 2, 3]. For the camera-ready version, we are happy to move the related work to the main text and make some experimental sections more concise by transferring their implementation details to the appendix, as also suggested by the reviewer VW9r.

@Artem, can you answer 5-11?


Reviewer VW9r:


1. However, unlike RNA seq, most of the geometric graphs do not come with an ordering. This means the proposed model is not for all "geometric graphs", it is for a small subset of "geometric graphs" where we have some ordering on the nodes. Thus the work do not comply with the main claim. The work may have a significant contribution to RNA-Seq analysis. However, as discussed earlier, in general cases, geometric graphs do not have order, thus severely limiting it's application.

We acknoweledge that GHyena requires ordering of the nodes and hence is applicable for a subset of geometric graphs such as biomolecules which naturally have this ordering. However, we strongly disagree with the reviewer that we did not mention this fact in the paper. Please see lines 422-435 in the main text under Limitations and Future work where we have explicitly dicussed this. Also please note that Reviewer YW9h mentions in their review that we have noted this limitation explicitly but we have also provided scenarios where this limitation can actually be beneficial (e.g.- in large biomolecules domain). Thus, we find the reviewer's comment somewhat unfair that we did not mention this limitation. We can highlght it more pronouncedly in the introduction of camera-ready version to make it more clear. Moreover, we would like to point out that the subset of geometric graphs for which our method is applicable is quite broad. For example, large biomolecules such as proteins, antibodies, RNA etc. which come with an ordering are extremely relevant for drug discovery. Also we submitted our paper under application track where biosciences is explicitly mentioned as an area under ICML call for papers (https://icml.cc/Conferences/2025/CallForPapers). Although other geometric graphs such as Point Clouds and meshes, etc. are undoubtedly important in several other domains, they are beyond the scope of our work as we focus on the equally important area of biomolecules (and especiually large biomolecules) and hence present our results for multiple RNA property prediction and protein molecular dynamics benchmarks. Finally, we would also like to point the reviewer to many recent and well-cited papers in NeurIPS, ICML, ICLR which focus solely on this important area [1, 2, 3] which the reviewer themselves acknoweldge that our proposed method can have a significant impact on RNA analysis. 


2. As claimed to be a generic model for Geometric data, authors should consider all the datasets from EQUIFORMER and VN-Transformer.
As explained in response to question 1, our work focuses primarily on biomolecues and graphs with ordering, the suugestion to run our model on datasets from VN-Transformer are not applicable (Model40 datasets is point cloud classification). Similarly, Equiformer uses small molecule dataset such as QM9 and MD17 which have few tens or hundreds of atoms. As the title of our paper says as well as explained in detail in the introduction, we focus on large scale datasets relevamnt for drug discovery (with thousands of nodes) where existing methods fail. None of the datasets in Equiformer or VNT are suitable for this. We hope that this clarifies that the datasets mentioned in Equiformer and VN-Transfomer paper are not relevant for our study. 

3. Also, as mentioned in line 307 -- "For the other models, we choose hyperparameters so their depth and total parameter count match those of Geometric Hyena, ensuring a fair comparison" --, It is not clear why it is not possible to use the hyper-parameters proposed in the original works.
VNT does not specify their optimal hyperparameters while EquiFormer default hyperparameters are tuned for the datsets that they considered. Furthermore, following reviewer's suggestion, we decided to run EquiFormer with the default hyperparameters and on A100 GPU with 81 GB GPU memory, Equiformer ran out of memory for all our datasets even with a batch size of 1. This goes on to also show why existing equivariant models are not suitable for large scale graphs such as large biomolecules (RNA, protein etc.) and also supplements our answers to questions 1 and 2 by the reviewer. Finally, our intital reason to run the models to match parameter count of GHyena was to ensure that we can fairly compare the benefits of these models by isolating the iompact of model scale on performance which is a standard practice [4, 5].

4. The experiments done are valid but not enough to demonstrate the significance.
We hope that the response to question 1 and 2 already clarifies the choice of our experiments. We have demonstrated significance of our method on 3 lareg-scale RNA property prediction tasks and 1 large-scale protein molecular dynamics task. The reviewers themselves acknwoledge that the proposed method can be a significant contribution for RNA data analysis which as rcenet papers in top ML conferences show are an important research area in itself. 

6. The idea of " Geometric associative recall" should be explained further. For example, the statement "In geometric associative recall, each bigram (key and value) is connected by a rotation matrix" is not well understood if not explained in more detail.
We will explain it here

7. Type line 241 ”Harry Potter” --> ``Harry Potter''
We will correct this!

8. Regarding "Vector long convolution," is this proposed by authors, or is it a standard definition?
Yes, this is a novel component of our model and we show that the vector long convolution can also be implemented efficiently in sub-quadeatic time. 



Response:
We thank the reviewer for their comments and questions. Below we answer them point-by-point.

**1. Claim for need of node ordering for GHyena:** We acknowledge that GHyena requires an ordering of the nodes, making it applicable to a subset of geometric graphs, such as biomolecules that naturally possess this ordering. However, we strongly disagree with the reviewer's assertion that we did not mention this fact in the paper. Specifically, we address this limitation explicitly in lines 422-435 of the main text under "Limitations and Future Work." Additionally, Reviewer YW9h notes that we have recognized this limitation while also providing scenarios where this could actually be beneficial, particularly in the domain of large biomolecules. Therefore, we believe the reviewer's comment regarding this is somewhat unfair. We are happy to highlight this limitation more prominently in the introduction of the camera-ready version to improve clarity. 

**2. Limited aplicability to RNA data only and Significance of Experiments:** The subset of geometric graphs applicable to our method is quite broad, including large biomolecules such as proteins, antibodies, and RNA, which are highly relevant for drug discovery. In addition to three RNA tasks (which the reviewer themselves acknowledge our method having a significant impact for), we have also showed the performance benefits of our method on even larger systems such as Protein Molecular Dynamics benchmark. The reviewer mentioned other geometric graphs, such as point clouds and meshes, which are indeed important in various domains but they fall outside the scope of our work, which emphasizes the equally crucial area of biomolecules (particularly large biomolecules).Please note that we submitted our paper under the application track, where biosciences is explicitly mentioned as a focus area in the ICML call for papers (https://icml.cc/Conferences/2025/CallForPapers). Lastly, we would like to direct the reviewer to several recent and well-cited papers published in NeurIPS, ICML, and ICLR that focus exclusively on this important area [1, 2, 3].

**3. Suggestion to Consider Datasets from EQUIFORMER and VN-Transformer:** As clarified in response to comment 2, our work is primarily focused on biomolecules and graphs with ordering. Therefore, the suggestion to run our model on datasets from VN-Transformer is not applicable, as the Model40 dataset is for point cloud classification. Similarly, Equiformer uses small molecule datasets such as QM9 and MD17, which involve only tens or hundreds of atoms. As stated in the title of our paper, as well as discussed in detail in the introduction, we concentrate on large-scale datasets relevant for drug discovery that consist of thousands of nodes, where existing methods struggle. None of the datasets from Equiformer or VN-Transformer are suitable for our study. We hope this explanation clarifies the relevance of the datasets mentioned in the Equiformer and VN-Transformer papers in relation to our research.

**4. Suggestion on Using Default Hyperparameters for Baselines:** We wish to clarify that VNT does not specify their optimal hyperparameters, while EquiFormer’s default hyperparameters are tuned for the datasets they considered. Still following the reviewer’s suggestion, we decided to run EquiFormer with its default hyperparameters on 8 A100 GPUs each with 81 GB of memory which we used for all our experiments. However, EquiFormer ran out of memory for all our datasets, even with a batch size of 1. This further illustrates why existing equivariant models are unsuitable for large-scale graphs like large biomolecules (RNA, protein, etc.) and complements our responses to Questions 1, 2 and 3, highlighting the importance of our work. Finally, our initial decision to match the parameter count of GHyena and baselines was aimed at ensuring a fair comparison by isolating the impact of model scale on performance, which is a standard practice [4, 5].


**5. Further Explanation of "Geometric Associative Recall:" 

**6. Correction of Typographical Error:** We will correct the typographical error regarding "Harry Potter" to ``Harry Potter'' as suggested.

**7. Clarification on "Vector Long Convolution:** To clarify, "Vector Long Convolution" is a novel component of our model. We also show that this convolution method can be implemented efficiently in sub-quadratic time.



Reviewer XkYv:

1. However, as the authors point out themselves, the performance benefit in the RNA property prediction task and on the geometric associative recall task is likely due to the alternating local and global context and not the long convolutions (the error bars for G-Transformer and G-Hyena overlap).

2. However, I am missing a baseline of a non-equivariant state space model (e.g. the non-equivariant Hyena model), since the claimed benefit of the proposed model is the combination of the efficiency state-space models with the performance of equivariant models. In light of recent doubts about the importance of equivariance (e.g. [arXiv.2311.17932], [arXiv: 2410.24169], AlphFold3) it would be interesting to see how the Geometric Hyena compares to efficient non-equivariant models.


3. There are numerous typos and grammatical errors in the manuscript (e.g. "Heyna" instead of "Hyena" in the tables). The related works section is an important part of the paper and has to be part of the main text, it does not belong in the supplementary material. For removing such an important section from the main text, the manuscript seems wordy at times, e.g. the "invariant-equivariant subspace interaction" section can be shortened considerably and the beginnings of sections 4.1 and 4.2 -> "implementation details" are almost the same. Also the equations given lack precision. For instance, the domain and co-domain of 
 given above (1) do not match the sets in (1) and the hatted quantities are not introduced. The notation 
 in (2) is not introduced. Similarly, the gating function 
 seems to act per token as it is introduced, is that correct?


Response:

**1. Misunderstanding Regarding Performance Benefits:** We believe there is a misunderstanding here. For the associative recall task specifically, we have observed that alternating local and global context alone is indeed sufficient for achieving the reported performance benefits. @Artem to expand

**2. Request for a Non-Equivariant State Space Model Baseline:** Thank you for this insightful point! In response to your suggestion, we have now conducted experiments with the vanilla non-equivariant Hyena model for both RNA property prediction and protein molecular dynamics tasks. We summarize our results below, which demonstrate that GHyena outperforms the non-equivariant counterparts across all tasks, with improvements ranging from 3% to 875%, depending on the specific task.

**3. Concerns About Typos and Grammatical Errors:**
We appreciate your feedback and will take the necessary steps to correct the typos and grammatical errors in the manuscript, including the incorrect spelling of "Hyena" in the tables. @Artem to address the rest.

**4. Related Works Section In Main Text:** We included the related works in the Appendix A due to page limitations. We followed the examples of prior works accepted at NeurIPS, ICML, and ICLR, which also compiled the related work in the appendix [1, 2, 3]. For the camera-ready version, we are happy to move the related work to the main text and make some experimental sections more concise by transferring their implementation details to the appendix.











==> rebuttal_response.tex <==
Thank you for acknowledging the practicality, effectiveness, and scalability of our method. We appreciate the reviewer's suggestion to emphasize the assumption of canonical ordering more explicitly, and we commit to making it more explicit in the camera-ready version. In addition to the edits in our previous response, we will :

- Rephrase paragraph 4 in the introduction (051R-063L) "... we propose Geometric Hyena that efficiently models global geometric context in sub-quadratic time while preserving equivariance to rotations and translations. In this work, we focus on a subset of geometric graphs where the canonical order can be established such as biomolecules. The focus on ordered geometric graphs differentiates Geometric Hyena from other equivariant frameworks. Having canonical ordering, we can leverage efficient sequence operators - long convolutions. For equivariance, we introduce vector long convolution that utilizes vector products ... "

- Rephrase the first contribution to "We propose Geometric Hyena, the first equivariant long-convolutional architecture specifically tailored for large geometric graphs with canonical ordering, designed to efficiently process global geometric context in sub-quadratic time."

- In 056R-061R, we will clarify: "The Geometric Hyena is designed for tasks that require modeling invariant and equivariant features in geometric graphs where canonical order can be established such as biomolecules [1]." 

- At the line 061R, we will add: "The canonical ordering of a geometric graph implies a unique and unambiguous enumeration of its nodes. For instance, in biomolecules, such canonical ordering is naturally established by IUPAC rules [1]. We refer to geometric graphs with canonical ordering as ordered geometric graphs."

- Will explicitly use sequence notation: "An ordered geometric graph of N nodes can be written as a sequence (x_1, f_1) ... (x_N, f_N)."


We believe that these modifications will address your concerns, and we are committed to improving the clarity based on your recommendations. We kindly request you to consider these revisions toward increasing your overall score!
